Identification over Poisson ISI Channels: Feedback and Molecular Applications

Molecular communication (MC) enables information transfer via molecules, making it ideal for biomedical applications where traditional methods fall short. In many such scenarios, identifying specific events is more critical than decoding full messages, motivating the use of deterministic identification (DI). This paper investigates DI over discrete-time Poisson channels (DTPCs) with inter-symbol interference (ISI), a realistic setting due to channel memory effects. We improve the known upper bound on DI capacity under power constraints from $\frac{3}{2} + \kappa$ to $\frac{1 + \kappa}{2}$. Additionally, we present the first results on deterministic identification with feedback (DIF) in this context, providing a constructive lower bound. These findings enhance the theoretical understanding of MC and support more efficient, feedback-driven biomedical systems.

==> Figures/table.tex <==
\begin{table}[H]
    \renewcommand{\arraystretch}{1.5} 
    \setlength{\tabcolsep}{6pt}
    \scalebox{0.75}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        $t$ & $1$ & $2$ & $\cdots$ & $K+1$ & $K+2$ & $K+3$ & $\cdots$ & $2(K+1)$ &$\cdots$ \\
        \hline
        $f_i^t$ & $\hat{E}$ & $0$ & $\cdots$ & $0$ & $\hat{E}$ & $0$ & $\cdots$ & $0$ & $\cdots$ \\
        \hline
        rate & $p_0\hat{E}T_s$ & $p_1\hat{E}T_s$ & $\cdots$ & $p_{K}\hat{E}T_s$ & $p_0\hat{E}T_s$ & $p_1\hat{E}T_s$ & $\cdots$ & $p_{K}\hat{E}T_s$ & $\cdots$ \\
        \hline
        $\boldsymbol{s}$ & \multicolumn{4}{c}{$\boldsymbol{s}_1$} & \multicolumn{4}{|c|}{$\boldsymbol{s}_2$} & $\cdots$ \\
        \hline
    \end{tabular}
    }
    \caption{Feedback encoding scheme and its corresponding rates of Poisson distributions of the channel outputs}
    \label{table:encdoing}
    \vspace{-1em}
\end{table}
